An Informative Tracking Benchmark

Along with the rapid progress of visual tracking, existing benchmarks become less informative due to redundancy of samples and weak discrimination between current trackers, making evaluations on all datasets extremely time-consuming. Thus, a small and informative benchmark, which covers all typical challenging scenarios to facilitate assessing the tracker performance, is of great interest. In this work, we develop a principled way to construct a small and informative tracking benchmark (ITB) with 7% out of 1.2 M frames of existing and newly collected datasets, which enables efficient evaluation while ensuring effectiveness. Specifically, we first design a quality assessment mechanism to select the most informative sequences from existing benchmarks taking into account 1) challenging level, 2) discriminative strength, 3) and density of appearance variations. Furthermore, we collect additional sequences to ensure the diversity and balance of tracking scenarios, leading to a total of 20 sequences for each scenario. By analyzing the results of 15 state-of-the-art trackers re-trained on the same data, we determine the effective methods for robust tracking under each scenario and demonstrate new challenges for future research direction in this field.

==> figures/screenshots-seqs-all.tex <==

\begin{figure*}[!htb]  
\renewcommand\arraystretch{1.0}
\setlength\tabcolsep{1pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ccccccccc}%{p{13cm} p{4cm}}
    \textbf{Human body}  & \textbf{Human part}    & \textbf{Animal}   & \textbf{Sign and logo}   & \textbf{Vehicle }   & \textbf{3D-object }     & \textbf{Sport ball}    & \textbf{UAV}   & \textbf{Cartoon} \\ 
            \includegraphics[width=0.11\linewidth]{./figures/seqs/skating.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs/hand.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/leopard.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/traffic-light.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/airplane.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/cube.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/basketball1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/drone.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/minis.png} \\ 
            %row 2
            \includegraphics[width=0.11\linewidth]{./figures/seqs/gym.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs/foot.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/panda.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/sign.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/boat.png} &
          \includegraphics[width=0.11\linewidth]{./figures/seqs/bottle.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/pingpang.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/uav-rocket.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/minions2019.png} \\ 
            %row 3
            \includegraphics[width=0.11\linewidth]{./figures/seqs/biker.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs/head.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/bee.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/night-speed.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/train-night.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/yoyo.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/volleyball.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/uav-f1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/jerry.png} \\ 
            %row 4
            \includegraphics[width=0.11\linewidth]{./figures/seqs/dancer.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs/head-boxing.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/flying-bird.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/stop-land.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/helicopter--.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/juggling.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/snooker.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/lake.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/Jerry2-2.png} \\ 
            %row 5
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/runner1.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/foot-breaking.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/butterflies.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/led-night-text.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/bike_auto.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/bottle-flip2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/basketball1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/eagle.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/kungfupanda3.png} \\ 
            %row 6
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/gym2.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/foot-dance3.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/cat-eat.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/led-snow-coke.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/bike-wild.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/box-inhand.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/basketball2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/air-ground-mbike2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs/kongfu.png} \\ 
            %row 7
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/high-jump.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/foot-disease1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/dogs.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-day-light1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/board.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/cup-inhand.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/golf1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/air-ground-skiing.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/croods1.png} \\ 
            %row 8
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/long-jump.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/foot-disease-2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/zebra.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-day-light2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/boat-racing.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/doll-train.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/golf2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/drone1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/thecroods0.png} \\ 
            %row 9
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/pairdiving.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/foot-run.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/panda-head.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-day-tunnel.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/bus.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/juggling1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/nineball.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/ground-air-drone2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/thecroods.png} \\ 
            %row 10
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/polevault.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/hand-ASL.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/dogs2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-mlines.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/car-drifting.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/moving-car3.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/pingpong.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/rocket3.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/lionKing.png} \\ 
    % Pedestrian &     Pedestrian   &   Pedestrian      &   Pedestrian  &   Pedestrian &  Pedestrian &  Pedestrian& Pedestrian  &Pedestrian       \\
    % Rider      &        &         &         &        &           &        &        &       \\
    % Pedestrian &        &         &         &        &           &        &        &       \\
    % Pedestrian &        &         &         &        &           &        &        &       \\
\end{tabular} }
\vspace{-2mm}
	\caption {\textbf{ Screenshots of the sequences from the first part of the proposed benchmark.} The sequences in every column belong to the same category whose name is given at the top. The target object in each sequence is annotated with a red (blur) bounding box. It shows that the target objects have a wide range of appearance and variation patterns which differ significantly.}
	\label{fig:screenshot-seqs-all-part1}
	\vspace{-2mm}
\end{figure*}



\begin{figure*}[!htb]  
\renewcommand\arraystretch{1.0}
\setlength\tabcolsep{1pt}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{ccccccccc}%{p{13cm} p{4cm}}
    \textbf{Human body}  & \textbf{Human part}    & \textbf{Animal}   & \textbf{Sign and logo}   & \textbf{Vehicle }   & \textbf{3D-object }     & \textbf{Sport ball}    & \textbf{UAV}   & \textbf{Cartoon} \\ 
            %row 1
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/Polo.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/hand-dance.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/LaSOT-goldfish-3.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-night-direction.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/car-night-driving.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/selfmoving-box.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/rugby1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/uav-car15.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/iceage1.png} \\ 
            %row 2
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/ski-jumping.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/hand-dance2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/LaSOT-shark-2.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/OTB-ClifBar.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/cars-racing.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/selfmoving-car.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/rugby2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/uav-car-drifting.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/iceage2.png} \\ 
            %row 3
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/NFS-basketball_7.jpg} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/hand-sign-1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/LaSOT-squirrel-13.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-night-light-3.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/jet-2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/selfmoving-car2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/rugbykick2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/uav-person19.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/insideout3.png} \\ 
            %row 4
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/NFS-parkour.jpg} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/head-breaking.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/NFS-dog_2.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-night-light4.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/moto-racing.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/toyinhand-yoyo.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/snooker2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/uav-uav4.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/insideout-face.png} \\ 
            %row 5
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/NFS-skydiving.jpg} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/head-football.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/butterfly-1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-night-rainy.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/train.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/toyself-moving.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/soccer.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/VisDrone-uav0000070_04877.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/my neighbor.png} \\ 
            %row 6
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/NUS-PRO-basketball_5.jpg} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/head-run.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/dolphin.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-night-yellow.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/train_goodview.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/doll-helicopter.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/soccer2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/VisDrone--uav0000080_01680_s.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/myneighbor1.png} \\ 
            %row 7
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/NUS-PRO-handball_4.jpg} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/head-swimming.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/air-ground-bull.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-snow-street.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/truck.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/LaSOT-kite-15.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/volleyball1.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/VisDrone--uav0000085_00000_s.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/walle.png} \\ 
            %row 8
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/NUS-PRO-soccer_6.jpg} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/LaSOT-hand_9.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/lion.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-street-speed.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/uav-bike3.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/LaSOT-robot-5.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/NFS-billiard_6.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/VisDrone--uav0000221_10400_s.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/wall-e.png} \\ 
            %row 9
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/OTB-Human3.jpg} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/LaSOT-hat2.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/fishs2.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/sign-text-coffee.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/LaSOT-motorcycle-18.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/NFS-airtable_3.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/NFS-pingpong_8.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/LaSOT-drone7.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/OTB-Bird1.jpg} \\ 
            %row 10
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanbody/pedestrian.png} & %\vspace{2mm}
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/humanpart/OTB-soccer.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/animals/bird-sea.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/signs-logos/LaSOT-licenceplate-12.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/vehicle/LaSOT-racing-20.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/3D-object/NFS-shuffletable_2.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/balls/LaSOT-vollecyball-13.jpg} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/uav/suv.png} &
            \includegraphics[width=0.11\linewidth]{./figures/seqs-others/cartoon/OTB_Ironman.jpg} \\ 
    % Pedestrian &     Pedestrian   &   Pedestrian      &   Pedestrian  &   Pedestrian &  Pedestrian &  Pedestrian& Pedestrian  &Pedestrian       \\
    % Rider      &        &         &         &        &           &        &        &       \\
    % Pedestrian &        &         &         &        &           &        &        &       \\
    % Pedestrian &        &         &         &        &           &        &        &       \\
\end{tabular} }
\vspace{-2mm}
	\caption {\textbf{Screenshots of the sequences from the second part of the proposed benchmark} The sequences in every column belong to the same category whose name is given at the top. The target object in each sequence is annotated with a red (blur) bounding box. It shows that the target objects have a wide range of appearance and variation patterns which differ significantly.}
	\label{fig:screenshot-seqs-all-part2}
	\vspace{-2mm}
\end{figure*}


% \begin{figure*}[!htb]   

% 		\begin{minipage}[c]{1\linewidth}
    		
%     		\setlength{\tabcolsep}{19.2mm}
%                 \begin{tabular}{c c c c c c c c c} 
%                      Human body& Human part & Animal & traffic sign & transportation & Doll  & sport ball & UAV & Cartoon  \\
%                 \end{tabular}
    
% 		\end{minipage}

% 		\begin{minipage}[c]{1\linewidth}
%             \includegraphics[width=0.11\linewidth]{./figures/seqs/soccer/6.png}   %\vspace{0.5mm}
% 			\includegraphics[width=0.11\linewidth]{./figures/seqs/soccer/68.png}
%             \includegraphics[width=0.11\linewidth]{./figures/seqs/soccer/76.png}
%             \includegraphics[width=0.11\linewidth]{./figures/seqs/soccer/136.png}
%             \includegraphics[width=0.11\linewidth]{./figures/seqs/soccer/260.png}
%             \includegraphics[width=0.11\linewidth]{./figures/seqs/soccer/327.png}
%             \includegraphics[width=0.11\linewidth]{./figures/seqs/soccer/327.png}
%             \includegraphics[width=0.11\linewidth]{./figures/seqs/soccer/327.png}
%             \includegraphics[width=0.11\linewidth]{./figures/seqs/soccer/327.png}
% 		\end{minipage}


% 	\caption {\textbf{Shots of some representative sequences in 9 scenarios.} }
% 	\label{fig:shot-seqs}
% \end{figure*}


==> tables/TB-rs-all.tex <==



\begin{table*}[t]
\begin{center}
\caption{\textbf{ Performance of all the 15 methods over each scenario and the overall benchmark in terms of the mIoU score (\%).} 
%
The last row shows the average score of all the 15 methods over each scenario. 
}
\label{Tab:results_all}
\vspace{-2mm}
\scriptsize
\renewcommand\arraystretch{1.1}
\setlength\tabcolsep{4pt}
 \resizebox{0.98\linewidth}{!}{
\begin{tabular}{l| ccccccccc c}
\toprule      
          \multicolumn{1}{r|}{Video set}
          &\multirow{2}{*}{\tabincell{c}{Human\\part}}
          &\multirow{2}{*}{\tabincell{c}{Sport\\ball}}
          &\multirow{2}{*}{\tabincell{c}{3D-\\object}}
          &\multirow{2}{*}{\tabincell{c}{Animal}}
          &\multirow{2}{*}{\tabincell{c}{UAV}}
          &\multirow{2}{*}{\tabincell{c}{Human\\body}}
          &\multirow{2}{*}{\tabincell{c}{Vehicle}}
          &\multirow{2}{*}{\tabincell{c}{Sign-and\\logo}}
          &\multirow{2}{*}{\tabincell{c}{Cartoon}}
          &\multirow{2}{*}{\tabincell{c}{Overall}}\\
        \multicolumn{1}{l|}{Method}  &&&&&&&&&&\\
\midrule
UDT~\cite{UDT}          &  18.86  &   9.67 &  26.23&   27.47 &   20.91 &  26.16 &  32.67&   63.47 &   44.46 &  29.99 \\
TADT~\cite{TADT}        &  30.68  &  27.14 &  30.09&   32.31 &   31.04 &   37.30 &  40.46&   64.25 &   49.59 &   38.10 \\
SiamRPN~\cite{SiamRPN}  &  29.27  &  25.86  &   32.73&    41.59 &  32.18 & 37.38 &  40.18&   48.97 &   57.95 &   38.46 \\
ECO~\cite{ECO}          &  40.54  & 26.52   &   39.28&   36.24 & 38.98 &   36.51  &  47.65&    65.24 &   61.49 &   43.61 \\
RPN++~\cite{SiamRPN++}  &  34.47  & 27.95  &  48.06&   45.90 &  37.27 &   45.65 & 49.30&    51.72 &  62.57 &  44.77 \\
SiamGAT~\cite{SiamGAT}  &  40.19  &  28.48   &  41.56&   47.84 &  32.63 &  43.17   & 52.49&   56.37 & 67.03 &   45.53 \\
Atom~\cite{ATOM}        &  36.36  & 33.28  &   46.42&    39.24 &  44.00 &   45.91 & 54.56&   66.91 &   66.42 &   48.12 \\
Ocean~\cite{OCEAN}      &   40.70  &  38.34  &   48.39&    47.37 &   41.42 &  52.28 & 55.79&   47.37 &  63.28 &  48.33 \\
KYS~\cite{KYS}          &   40.78  &  46.29  &  51.37&   47.78 &   48.59 &  50.10 & 54.01&   67.37 &   69.52 &  52.87 \\
DiMP~\cite{DiMP}        &   38.57  &  51.49  &   46.45&    47.89 &   55.17 &   49.32 &  63.51&    65.67 &   69.38 &  54.16 \\
PrDiMP~\cite{PrDiMP}    &   40.14  & 51.77  &  47.16&   49.66 &  53.38 &   56.11 &  62.47&    66.32 &  69.65 &   55.19 \\
TransT~\cite{TransT}    &   44.04  &  40.78  &  54.73&  50.76 &  59.46 &   66.63 &  63.53&    52.09 &   66.98 &   55.45 \\
LTMU~\cite{LTMU}        &   42.80  &  48.45  &  47.44&    50.31 &   59.04 &   56.22 &  66.71&   70.09 &  69.46 &  56.72 \\
TrDiMP~\cite{TrDiMP}    &   39.55  &  53.32  &  49.98&   54.38 &  62.63 &   56.44 & 66.21&    62.94 &  69.07 &   57.17 \\
Stark~\cite{Stark}      &   41.49  & 51.05  &  53.96&    55.55 &  63.47 &   66.72 &  65.80&    59.19 &  69.09 &   58.48 \\ \midrule
Average                 &   37.23  & 37.36  &  44.26&    44.95 &  45.35 &   48.39 &  54.36&    60.53 &  63.73 &   48.46 \\
\bottomrule
\end{tabular}}
\end{center}
\vspace{-4mm}
\end{table*}



% this version contains the std score
% \begin{table*}[t]
% \begin{center}
% \caption{\textbf{ Performance of 10 state-of-the-art methods on ITB and all benchmarks, and the comparisons between them in terms of challenge degree, discriminant ability, and evaluation efficiency.} 
% %
% The left part shows the mIoU scores of each method on each benchmark and the right part compares the stats of mean mIoU, normalized std (NStd, computed by dividing std by mean mIoU), and test time (minute) for each dataset.
% %
% }
% \label{Tab:overall_results}
% \vspace{-2mm}
% \scriptsize
% \renewcommand\arraystretch{1.1}
% \setlength\tabcolsep{4pt}
%  \resizebox{0.95\linewidth}{!}{
% \begin{tabular}{l| cccccccccc|cccr}
% \toprule      
%           \multicolumn{1}{r|}{Trackers }&\multicolumn{3}{c|}{Siamese} &\multicolumn{4}{c|}{Classifier+IoUNet} &\multicolumn{3}{c|}{Transformer} &\multirow{2}{*}{\tabincell{c}{mean\\mIoU }} &\multirow{2}{*}{\tabincell{c}{Std\\mIoU }} &\multirow{2}{*}{\tabincell{c}{NStd\\mIoU }}&\multirow{2}{*}{\tabincell{c}{Test\\time} }\\
% Datasets & RPN++ & Ocean & \multicolumn{1}{c|}{GAT} & ATOM  & DiMP  & PrDiMP  & \multicolumn{1}{c|}{KYS}   & TrDiMP &TransT &Stark & & & &\\
% \midrule
% OTB100  & 66.6 & 65.6 & 65.3 & 65.6 & 67.4 & 68.7 & 69.4 & 69.7 & 67.0 & 69.0 & 67.4  & 1.67 & 2.40 & 41m \\
% NUS-PRO & 53.1 & 56.7 & 52.7 & 56.6 & 59.1 & 59.2 & 60.5 & 60.2 & 62.8 & 62.4 & 58.3  & 3.51 & 5.59& 94m \\
% UAV123  & 57.8 & 58.3 & 59.1 & 63.2 & 64.8 & 66.7 & 63.7 & 65.4 & 65.5 & 68.6 & 63.3  & 3.72 & 5.42& 78m \\
% VisDrone& 57.2 & 63.1 & 54.5 & 57.4 & 61.1 & 54.8 & 61.6 & 62.5 & 60.7 & 60.2 & 59.3  & 3.11 & 4.94& 53m \\
% NFS(30) & 49.7 & 54.3 & 52.6 & 58.8 & 62.4 & 62.9 & 62.9 & 64.1 & 63.6 & 65.6 & 59.7  & 5.55 & 8.46& 33m\\
% TNet    & 69.0 & 69.2 & 71.7 & 72.5 & 74.9 & 75.8 & 74.1 & 78.3 & 80.7 & 81.1 & 74.7  &4.32& 5.33& 156m\\
% Got10K  & 48.8 & 59.9 & 53.8 & 56.1 & 61.4 & 64.6 & 62.1 & 68.2 & 70.2 & 68.8 & 61.2  &  6.96& 9.91& 16m\\
% LaSOT   & 49.2 & 55.2 & 51.0 & 51.0 & 57.4 & 60.8 & 53.4 & 62.4 & 65.5 & 66.3 & 57.2   & 6.25 & 9.42& 476m\\ \hline
% ITB (ours)  & 44.1 & 47.7 & 44.9 & 47.2 & 53.7 & 54.4 & 52.0 & 56.1 & 54.7 & 57.6 & 51.2 & 4.86 & 8.44& 60m \\
% \bottomrule
% \end{tabular}}
% \vspace{-4mm}
% \end{center}
% \end{table*}


% % containing eco udt tadt rpn ltmu.
% \begin{table*}[t]
% \begin{center}
% \caption{\textbf{ Comparison of TinyTB against existing benchmarks in terms of difficulty, discriminant ability, and efficiency.} }
% \label{Tab:datasets}
% %\vspace{1mm}
% \scriptsize
% \renewcommand\arraystretch{1.2}
% \setlength\tabcolsep{4pt}
%  \resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l| ccccccccccccccc }
% \toprule      
%           \multicolumn{1}{r|}{Trackers }  &\multicolumn{3}{c|}{Others}&\multicolumn{5}{c|}{Siamese}&\multicolumn{4}{c|}{Classifier+IoUNet}&\multicolumn{3}{c}{Transformer }\\
% Datasets &  ECO & UDT & LTMU   & RPN & TADT & RPN++ & Ocean & GAT    & ATOM  & DiMP  & PrDiMP  & KYS  & TrDiMP &TransT &Stark   \\
% \midrule
% OTB100  & 0.666&0.552& 0.680  &0.615& 0.646&0.666  & 0.656 & 0.653  & 0.656 & 0.674 & 0.687   &0.694 & 0.697  & 0.670  & 0.690   \\
% NUS-PRO & 0.551&0.426& 0.617  &0.490& 0.513 &0.531 & 0.567 &  0.527 & 0.566 &  0.591& 0.592   & 0.605&0.602   & 0.628  & 0.624   \\
% UAV123  & 0.537&0.463& 0.506  &0.551&0.502  & 0.578& 0.583 & 0.591  & 0.632 &0.648  & 0.667   &0.637 &0.654   &0.655   & 0.686   \\
% VisDrone& 0.526&0.457& 0.569  &0.502&0.525  &0.572 & 0.631 & 0.545  & 0.574 & 0.611 & 0.548   & 0.616& 0.625  &0.607   & 0.602   \\
% NFS     &0.520 & 0.322&0.643  &0.453& 0.456 & 0.497&0.543  &  0.526 &  0.588&0.624  & 0.629   &  0.629& 0.641 & 0.636  & 0.656   \\
% TNet    &   &    &       &    &    &    &  &     &   &     &         &    &  &   &       \\
% Got10K & 0.417& 0.235& 0.667 & 0.397 &0.355& 0.488&0.599  & 0.538  &0.561  & 0.614 & 0.646   &0.621  &0.682     &0.702   & 0.688    \\
% LaSOT   & 0.365& 0.253 & 0.645&0.411  &0.331& 0.492& 0.552 &0.510   & 0.510 & 0.574 & 0.608   &0.534  & 0.624 & 0.655  &  0.663   \\
% TinyTB  &       &        &       &   &   &    &  &     &      &     &      &    &  &   &       \\
% \bottomrule
% \end{tabular}}
% \end{center}
% \end{table*}

% \begin{table*}[t]
% \begin{center}
% \caption{\textbf{ Comparison of TinyTB against existing benchmarks in terms of difficulty, discriminant ability, and efficiency.} }
% \label{Tab:datasets}
% %\vspace{1mm}
% \scriptsize
% \renewcommand\arraystretch{1.1}
% \setlength\tabcolsep{4pt}
%  \resizebox{0.95\linewidth}{!}{
% \begin{tabular}{l| ccccccccc   ccc }
% \toprule
%     \multicolumn{1}{r|}{-}        & \multicolumn{9}{c}{Benchmarks (AUC score)} & \multirow{2}{*}{\tabincell{c}{Challenge\\degree} }&\multirow{2}{*}{\tabincell{c}{Std} }&\multirow{2}{*}{\tabincell{c}{Efficiency} }\\
% trackers         & OTB100  & NUS-PRO& UAV123    & VisDrone   & NFS & TNet & Got-10K   &   LaSOT     & TinyTB &   &   &  \\ \midrule
% ECO       &66.6   &55.1  &53.7       &52.6     &52.0   &       &41.7            &36.5         &    &  &   &       \\
% UDT       &55.2   &42.6  &46.3       &45.7     &32.2   &       &23.5            &25.3         &    &  &   &       \\
% LTMU      &68.0   &61.7  &50.6       &56.9     &64.3   &       &66.7            &64.5         &    &  &   &       \\
% RPN       &61.5   &49.0  &55.1       &50.2     &45.3   &       &39.7            &41.1         &    &  &   &       \\
% TADT      &64.6   &51.3  &50.2       &52.5     &45.6   &       &35.5            &33.1         &    &  &   &       \\
% RPN++     &66.6   &53.1  &57.8       &57.2     &49.7   &       &48.8            &49.2         &    &  &   &       \\
% Ocean     &65.6   &56.7  &58.3       &63.1     &54.3   &       &59.9            &55.2         &    &  &   &       \\
% SiamGAT   &65.3   &52.7  &59.1       &54.5     &52.6   &       &53.8            &51.0         &    &  &   &       \\
% ATOM      &65.6   &56.6  &63.2       &57.4     &58.8   &       &56.1            &51.0         &    &  &   &       \\
% DiMP      &67.4   &59.1  &64.8       &61.1     &62.4   &       &61.4            &57.4         &    &  &   &       \\
% PrDiMP    &68.7   &59.2  &66.7       &54.8     &62.9   &       &64.6            &60.8         &    &  &   &       \\
% KYS       &69.4   &60.5  &63.7       &61.6     &62.9   &       &62.1            &53.4         &    &  &   &       \\
% TrDiMP    &69.7   &60.2  &65.4       &62.5     &64.1   &       &            &62.4         &    &  &   &       \\
% TransT    &67.0   &62.8  &65.5       &60.7     &63.6   &       &70.2            &65.5         &    &  &   &       \\
% Stark     &69.0   &62.4  &68.6       &60.2     &65.6   &       &68.8            &66.3         &    &  &   &       \\
% \bottomrule
% \end{tabular}}
% \end{center}
% \end{table*}


% \begin{table*}[t]
% \begin{center}
% \caption{\textbf{Comparison of TinyTB against existing datasets.} }
% \label{Tab:datasets}
% %\vspace{1mm}
% \scriptsize
% \renewcommand\arraystretch{1.3}
% \setlength\tabcolsep{4pt}
%  \resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l| r r r r r r r r r   r r r }
% \toprule
%     \multicolumn{1}{r|}{Info.}        & \multicolumn{9}{c|}{Scenarios} & \multicolumn{3}{c}{Status}\\
% Dataset            & Human body & Human part & Animal  & Vehicle & Traffic signs & Sport balls &     Doll   &   UAV     & Cartoon & Scenario Nb & Video number & Total frames\\ \midrule
            
% OTB2015    & 36 / 10 & 26 / 3  & 3 / 3   &  14 / 3   &  3 / 3  &    0 / 0  & 16 / 10  &  0 / 0    &  2 / 1    & 7  & 100  & 59K    \\
% VOT-2020   & 15 / 8       &  12 / 3   & 14 / 11          &  4 / 4            &  7 / 7             & 3 / 3              &   2 / 2        &    3 / 1       & 0 / 0     & 8  & 60   &  21.3K  \\
% NUS-PRO    & 205 / 6      &   60 / 1        & 0 / 0    &  100 / 5      &   0 / 0       &  0 / 0    &  0 / 0   &   0 / 0   &  0 / 0     & 3  & 365  & 135K       \\
% UAV123     &  0 / 0          &   0 / 0         &  0 / 0          &    0 / 0            &     0 / 0           &        0 / 0        &   0 / 0         &  123 / 2         &  0 / 0     & 1  & 123  &  113K      \\
% VisDrone   &  0 / 0          &   0 / 0         &  0 / 0          &    0 / 0            &     0 / 0           &        0 / 0        &   0 / 0         &  97 / 1         &  0 / 0     & 1  & 97  &  76K      \\
% NFS        & 20 / 11          &  6 / 4         & 14 / 7          &  15 / 6             &  5 / 5             &  22 / 6             &  17 / 7         &   1 / 1        & 0 / 0    &  8  & 100    &   383K    \\
% LaSOT      &  4 / 4         & 12 / 3           &   136 / 34        &  40 / 10             &   4 / 1            &  12 /3             &  64 / 16         & 4 / 1          &  4 / 4     & 9   & 280    & 685K  \\
% TrackingNet&  131 / 11         &   4 / 1        & 151 / 18          &  158 / 9             &   0 / 0            &   0 / 0            &   65 / 6        &   0 / 0        & 0 / 0    &  5 & 511    &  225K     \\
% Got-10K    & 30 / 7          &  0 / 0         & 109 / 28          &   22 / 5            &  0 / 0             &  0 / 0            &  19 / 5         &   0 / 0        & 0 / 0     & 4  & 180    & 23K       \\ \midrule
% TinyTB    &    20/       &    20/       &     20/       &       20/         &   20/             &      20/          &        20/    &     20/       &   20/   & 9/  &  180  &  98K      \\
% \bottomrule


% \end{tabular}}
% \end{center}

% \end{table*}

==> tables/seq-details.tex <==



% \begin{table*}[t]
% \begin{center}
% \caption{\textbf{ Detailed information about each sequence.} }
% \label{Tab:seq-info}
% \vspace{-2mm}
% \renewcommand\arraystretch{1.1}
% \setlength\tabcolsep{4pt}
 
\begin{longtable}{ll| cccccccc}
\caption{\textbf{ Detailed information of the 180 sequences.} Length: frame number of a sequence, Mean-IoU: mean IoU score obtained by the 15 methods given in the manuscript }
\label{Tab:seq-info}\\
%  \resizebox{0.98\linewidth}{!}{

\toprule    
          &\multicolumn{1}{l|}{Sequence name}
          &\multirow{1}{*}{\tabincell{c}{Length}}
          &\multirow{1}{*}{\tabincell{c}{Mean-IoU}}
          &\multirow{1}{*}{\tabincell{c}{STD-IoU}}
          &\multirow{1}{*}{\tabincell{c}{Var-density}}
          &\multirow{1}{*}{\tabincell{c}{Quality}}
          &\multirow{1}{*}{\tabincell{c}{Source}}
          &\multirow{1}{*}{\tabincell{c}{Challenges}}
          &\multirow{1}{*}{\tabincell{c}{Sce.}}\\
\midrule

%--Human part
\multirow{20}{*}{\rotatebox{90}{Human part}}&hand-piano 	     & 204 & 0.623 & 0.177 & 1.065 &0.570 & new & \\
foot-running 	 & 117 & 0.592 & 0.238 & 0.953 &0.577 & new& \\
helmet-football  & 284 & 0.485 & 0.103 & 1.039 &0.676 & new& \\
foot-dance   	 & 352 & 0.502 & 0.142 & 1.068 &0.680 & new& \\
helmet           & 125 & 0.565 & 0.302 & 1.090 &0.700 & new& \\
head-men's100 	 & 134 & 0.519 & 0.167 & 1.053 &0.718 & new& \\
foot-gait-1 	 & 245 & 0.454 & 0.116 & 0.956 &0.742 & new& \\
foot-gait-2 	 & 235 & 0.319 & 0.098 & 0.731 &0.863 & new& \\
head-breaking2 	 & 230 & 0.370 & 0.144 & 1.044 &0.865 & new& \\
head-swimming 	 & 175 & 0.371 & 0.138 & 0.995 &0.885 & new& \\
hand-ASL         & 398 & 0.424 & 0.193 & 0.977 &0.891 & new& \\
Soccer 	         & 392 & 0.335 & 0.113 & 0.771 &0.893 & OTB2015& \\
foot-ballet 	 & 336 & 0.066 & 0.041 & 1.056 &0.897 & new& \\
hand-language2 	 & 144 & 0.311 & 0.117 & 1.106 &0.904 & new& \\
hand-dance-1 	 & 357 & 0.264 & 0.160 & 1.051 &0.969 & new& \\
hand-dance-2 	 & 342 & 0.310 & 0.175 & 1.082 &0.971 & new& \\
foot-breaking 	 & 193 & 0.181 & 0.107 & 1.121 &1.022 & new& \\
hat-2 	         & 1461 & 0.361 & 0.216 & 1.031 &1.025 & LaSOT& \\
head-boxing 	 & 297 & 0.247 & 0.264 & 1.081 &1.049 & new& \\
hand-9 	         & 1733 & 0.144 & 0.085 & 0.870 &1.087 & LaSOT& \\ \midrule
%--Sport ball
soccer 2 	 & 77 & 0.715 & 0.191 & 1.160 &0.420 & new& \multirow{20}{*}{\tabincell{c}{Sport\\ball}}\\
basketball-3 & 130 & 0.619 & 0.136 & 1.128 &0.444 & new& \\
rugby 1 	 & 109 & 0.610 & 0.226 & 0.976 &0.572 & new& \\
rugby-kick2 	 & 100 & 0.219 & 0.045 & 1.074 &0.611 & new& \\
basketball-1 	 & 118 & 0.599 & 0.304 & 1.023 &0.629 & new& \\
valleyball1 	 & 281 & 0.547 & 0.322 & 1.009 &0.832 & new& \\
golf 2 	 & 153 & 0.395 & 0.189 & 1.091 &0.861 & new& \\
volleyball 	 & 142 & 0.131 & 0.162 & 1.132 &0.865 & new& \\
snooker-2 	 & 88 & 0.195 & 0.285 & 0.999 &0.881 & new& \\
rugby 2 	 & 166 & 0.390 & 0.191 & 0.979 &0.886 & new& \\
nine-ball-pool 	 & 210 & 0.456 & 0.320 & 0.940 &0.886 & new& \\
basketball-2 	 & 123 & 0.385 & 0.256 & 1.018 &0.913 & new& \\
snooker-1 	 & 98 & 0.310 & 0.330 & 1.075 &0.934 & new& \\
pingpong-8 	 & 296 & 0.186 & 0.129 & 1.046 &0.987 & NFS& \\
golf 1 	 & 138 & 0.353 & 0.292 & 0.950 &1.043 & new& \\
pingpang 2 	 & 103 & 0.230 & 0.246 & 0.942 &1.064 & new& \\
Ping Pong 	 & 107 & 0.223 & 0.290 & 1.038 &1.099 & new& \\
soccer 	 & 225 & 0.303 & 0.262 & 1.079 &1.112 & new& \\
billiard-6 	 & 771 & 0.349 & 0.365 & 0.990 &1.114 & NFS& \\
volleyball-13 	 & 2004 & 0.255 & 0.295 & 1.166 &1.292 & LaSOT& \\\midrule
%--3D-object
toy-car1 	 & 201 & 0.759 & 0.124 & 0.840 &0.299 & new& \multirow{20}{*}{\tabincell{c}{3D-\\object}}\\
yoyo-inhand-night 	 & 321 & 0.749 & 0.054 & 1.013 &0.320 & new& \\
toy-car3 	 & 409 & 0.662 & 0.088 & 1.095 &0.376 & new& \\
toy-fight 	 & 256 & 0.715 & 0.172 & 1.159 &0.396 & new& \\
toy-train 	 & 380 & 0.653 & 0.112 & 1.158 &0.405 & new& \\
box-inhand 	 & 438 & 0.667 & 0.137 & 1.022 &0.416 & new& \\
cubes-inhand 	 & 149 & 0.626 & 0.180 & 1.063 &0.460 & new& \\
bottle-flip2 	 & 136 & 0.619 & 0.218 & 1.010 &0.564 & new& \\
toy-helicopter 	 & 400 & 0.559 & 0.152 & 1.006 &0.612 & new& \\
cup-inhand 	 & 418 & 0.142 & 0.054 & 0.915 &0.718 & new& \\
toy-car2 	 & 268 & 0.461 & 0.215 & 0.714 &0.786 & new& \\
bottle-flip 	 & 127 & 0.425 & 0.245 & 1.071 &0.812 & new& \\
toy-box 	 & 479 & 0.278 & 0.175 & 1.114 &0.882 & new& \\
toy-inhand-yoyo 	 & 404 & 0.461 & 0.290 & 0.986 &0.922 & new& \\
juggling-2 	 & 168 & 0.121 & 0.055 & 1.031 &0.935 & new& \\
robot-5 	 & 2267 & 0.290 & 0.159 & 0.981 &0.947 & LaSOT& \\
juggling-1 	 & 211 & 0.094 & 0.074 & 1.084 &1.006 & new& \\
shuffletable-2 	 & 372 & 0.262 & 0.267 & 0.979 &1.063 & NFS& \\
airtable-3 	 & 482 & 0.152 & 0.176 & 0.962 &1.083 & NFS& \\
kite-15 	 & 2064 & 0.156 & 0.202 & 0.996 &1.290 & LaSOT& \\\midrule
%--Animal
Panda-head 	 & 312 & 0.746 & 0.076 & 1.000 &0.303 & new& \multirow{20}{*}{\tabincell{c}{Animal}}\\
leopard 	 & 221 & 0.710 & 0.114 & 1.100 &0.366 & new& \\
horse-zebra 	 & 286 & 0.596 & 0.099 & 1.174 &0.483 & new& \\
lion-running 	 & 367 & 0.666 & 0.215 & 1.061 &0.494 & new& \\
air-sea-dolphin 	 & 342 & 0.610 & 0.156 & 1.001 &0.494 & new& \\
cat-eat 	 & 381 & 0.564 & 0.074 & 0.919 &0.507 & new& \\
butterfly-2 	 & 302 & 0.647 & 0.162 & 0.965 &0.536 & new& \\
panda-funny 	 & 383 & 0.567 & 0.164 & 0.976 &0.597 & new& \\
bird-flying 	 & 440 & 0.574 & 0.174 & 0.894 &0.648 & new& \\
dogs 	 & 395 & 0.402 & 0.148 & 1.041 &0.754 & new& \\
bull 	 & 131 & 0.401 & 0.210 & 0.781 &0.772 & new& \\
bird-sea 	 & 378 & 0.384 & 0.197 & 0.990 &0.873 & new& \\
fish2 	 & 371 & 0.355 & 0.223 & 0.975 &0.915 & new& \\
bee-group 	 & 431 & 0.377 & 0.252 & 1.129 &0.958 & new& \\
squirrel-13 	 & 1927 & 0.214 & 0.099 & 1.112 &1.013 & LaSOT& \\
dogs2 	 & 394 & 0.320 & 0.194 & 1.182 &1.026 & new& \\
dog-2 	 & 594 & 0.129 & 0.202 & 1.041 &1.084 & NFS& \\
shark-2 	 & 3441 & 0.235 & 0.147 & 1.091 &1.113 & LaSOT& \\
butterfly-1 	 & 305 & 0.270 & 0.249 & 0.968 &1.157 & new& \\
goldfish-3 	 & 2163 & 0.225 & 0.168 & 0.973 &1.204 & LaSOT& \\\midrule
%--UAV
air-ground-f1 	 & 241 & 0.693 & 0.180 & 0.938 &0.361 & new& \multirow{20}{*}{\tabincell{c}{UAV}}\\
air-ground-bike-2 	 & 361 & 0.729 & 0.208 & 1.125 &0.402 & new& \\
air-ground-lake 	 & 321 & 0.668 & 0.184 & 1.091 &0.424 & new& \\
ground-air-drone1 	 & 584 & 0.658 & 0.194 & 0.940 &0.494 & new& \\
ground-air-drone2 	 & 347 & 0.592 & 0.130 & 1.034 &0.519 & new& \\
skating-uav 	 & 319 & 0.602 & 0.111 & 1.113 &0.520 & new& \\
air-ground-skiing 	 & 462 & 0.527 & 0.156 & 0.954 &0.671 & new& \\
air-ground-car 	 & 554 & 0.553 & 0.214 & 1.055 &0.677 & new& \\
air-air-rocket3 	 & 158 & 0.576 & 0.270 & 1.053 &0.685 & new& \\
air-air-rocket4 	 & 926 & 0.422 & 0.180 & 0.825 &0.800 & new& \\
air-air-drone1 	 & 463 & 0.364 & 0.156 & 1.107 &0.870 & new& \\
air-air-eagle 	 & 387 & 0.450 & 0.296 & 0.965 &0.954 & new& \\
uav0000080-01680-s 	 & 1201 & 0.335 & 0.211 & 1.123 &0.986 & VisDrone& \\
uav0000070-04877-s 	 & 332 & 0.278 & 0.229 & 0.971 &0.997 & VisDrone& \\
person19-3 	 & 1567 & 0.297 & 0.216 & 0.898 &1.002 & UAV& \\
car15 	 & 469 & 0.387 & 0.279 & 1.039 &1.043 & UAV& \\
uav0000085-00000-s 	 & 1645 & 0.264 & 0.233 & 0.949 &1.086 & VisDrone& \\
uav0000221-10400-s 	 & 2970 & 0.159 & 0.226 & 1.049 &1.120 & VisDrone& \\
uav4 	 & 157 & 0.204 & 0.192 & 0.946 &1.125 & UAV& \\
drone-7 	 & 2708 & 0.313 & 0.257 & 1.045 &1.196 & LaSOT& \\\midrule
%--Human body
mountain-biker 	 & 226 & 0.656 & 0.135 & 1.161 &0.408 & new& \multirow{20}{*}{\tabincell{c}{Human\\body}}\\
long-jump 	 & 298 & 0.719 & 0.163 & 1.104 &0.410 & new& \\
polo 	 & 301 & 0.637 & 0.064 & 1.119 &0.419 & new& \\
beark-dancer 	 & 357 & 0.702 & 0.135 & 1.054 &0.425 & new& \\
pole-vault 	 & 199 & 0.642 & 0.116 & 1.032 &0.478 & new& \\
high-jumper 	 & 300 & 0.632 & 0.153 & 1.207 &0.507 & new& \\
ski-jumper 	 & 315 & 0.575 & 0.144 & 1.110 &0.517 & new& \\
pedestrian 	 & 147 & 0.523 & 0.099 & 1.003 &0.518 & new& \\
skater2 	 & 319 & 0.602 & 0.111 & 0.985 &0.520 & new& \\
runner1 	 & 192 & 0.559 & 0.145 & 1.168 &0.642 & new& \\
pair-diving 	 & 60 & 0.534 & 0.196 & 1.083 &0.661 & new& \\
gymnastics3 	 & 380 & 0.569 & 0.224 & 1.158 &0.734 & new& \\
gymnastics2 	 & 300 & 0.574 & 0.311 & 1.078 &0.753 & new& \\
Human3 	 & 1698 & 0.506 & 0.294 & 0.938 &0.908 & OTB2015& \\
parkour 	 & 58 & 0.146 & 0.159 & 1.066 &0.910 & NFS& \\
basketball-7 	 & 240 & 0.327 & 0.227 & 1.175 &0.947 & NFS& \\
basketball-005 	 & 196 & 0.218 & 0.138 & 1.105 &0.975 & NUS-PRO& \\
Skydiving 	 & 196 & 0.213 & 0.147 & 1.097 &0.993 & NFS& \\
handball-004 	 & 218 & 0.202 & 0.174 & 1.077 &0.994 & NUS-PRO& \\
soccer-006 	 & 387 & 0.143 & 0.214 & 1.059 &1.017 & NUS-PRO& \\\midrule
%--Vehicle
car-night 	 & 422 & 0.793 & 0.039 & 1.110 &0.246 & new&\multirow{20}{*}{\tabincell{c}{Vehicle}}\\
bike-wild 	 & 205 & 0.763 & 0.122 & 1.094 &0.284 & new& \\
bike-auto 	 & 390 & 0.725 & 0.120 & 0.970 &0.313 & new& \\
car-drifting 	 & 460 & 0.761 & 0.246 & 1.062 &0.338 & new& \\
cars-racing 	 & 248 & 0.657 & 0.084 & 1.144 &0.393 & new& \\
motor-racing 	 & 392 & 0.651 & 0.136 & 1.135 &0.418 & new& \\
train-night 	 & 449 & 0.699 & 0.251 & 1.015 &0.445 & new& \\
plane-takingoff 	 & 472 & 0.572 & 0.103 & 1.192 &0.488 & new& \\
board 	 & 392 & 0.612 & 0.134 & 1.070 &0.491 & new& \\
train-1 	 & 317 & 0.556 & 0.121 & 1.167 &0.514 & new& \\
boat-racing2 	 & 349 & 0.620 & 0.228 & 1.035 &0.551 & new& \\
boat-racing1 	 & 450 & 0.597 & 0.219 & 1.052 &0.615 & new& \\
helicopter1 	 & 425 & 0.597 & 0.249 & 0.960 &0.624 & new& \\
truck 	 & 402 & 0.564 & 0.171 & 0.892 &0.627 & new& \\
jet-2 	 & 388 & 0.486 & 0.247 & 1.121 &0.733 & new& \\
suv 	 & 457 & 0.239 & 0.090 & 1.106 &0.901 & new& \\
train-highspeed 	 & 407 & 0.302 & 0.219 & 1.058 &0.973 & new& \\
bike3 	 & 433 & 0.302 & 0.203 & 1.081 &0.995 & UAV& \\
racing-20 	 & 2812 & 0.167 & 0.174 & 0.996 &1.088 & LaSOT& \\
motorcycle-18 	 & 2382 & 0.209 & 0.254 & 1.060 &1.243 & LaSOT& \\\midrule
%--Sign and logo
led-snowy-coke 	 & 350 & 0.837 & 0.069 & 1.173 &0.166 & new& \multirow{20}{*}{\tabincell{c}{Sign-and\\-logo}}\\
sign-night-yellow 	 & 267 & 0.827 & 0.065 & 1.058 &0.200 & new& \\
sign-day-tunnel 	 & 294 & 0.797 & 0.073 & 1.216 &0.239 & new& \\
sign-night-direction 	 & 305 & 0.786 & 0.054 & 1.049 &0.257 & new& \\
sign-night-led 	 & 399 & 0.758 & 0.065 & 0.979 &0.290 & new& \\
sign-night-speed 	 & 219 & 0.742 & 0.056 & 1.164 &0.295 & new& \\
text-mlines 	 & 225 & 0.735 & 0.229 & 1.144 &0.356 & new& \\
sign-day-light1 	 & 348 & 0.715 & 0.128 & 1.036 &0.364 & new& \\
sign-snow-street 	 & 385 & 0.677 & 0.078 & 1.106 &0.387 & new& \\
sign-day-direction2 	 & 226 & 0.659 & 0.124 & 0.990 &0.414 & new& \\
sign-day-light2 	 & 187 & 0.661 & 0.175 & 1.054 &0.458 & new& \\
sign-street-speed 	 & 235 & 0.621 & 0.216 & 1.031 &0.568 & new& \\
sign-night-light4 	 & 185 & 0.467 & 0.124 & 1.117 &0.574 & new& \\
text-coffee 	 & 188 & 0.588 & 0.279 & 1.014 &0.577 & new& \\
sign-night-light 	 & 353 & 0.492 & 0.126 & 1.108 &0.716 & new& \\
sign-night-light3 	 & 357 & 0.423 & 0.151 & 0.915 &0.740 & new& \\
clifBar 	 & 472 & 0.484 & 0.182 & 1.011 &0.786 & OTB2015& \\
sign-groundstop 	 & 77 & 0.286 & 0.206 & 0.950 &0.868 & new& \\
led-night-text 	 & 295 & 0.285 & 0.293 & 1.036 &1.064 & new& \\
licenseplate-12 	 & 2554 & 0.267 & 0.179 & 1.007 &1.076 & LaSOT& \\\midrule
%--Cartoon
insideout-face 	 & 299 & 0.803 & 0.045 & 0.935 &0.223 & new& \multirow{20}{*}{\tabincell{c}{Cartoon}}\\
Wall-E-1 	 & 320 & 0.744 & 0.093 & 1.123 &0.287 & new& \\
tom-jerry-1 	 & 227 & 0.744 & 0.042 & 1.143 &0.297 & new& \\
Totoro1 	 & 379 & 0.734 & 0.093 & 1.012 &0.303 & new& \\
Totoro0 	 & 351 & 0.747 & 0.221 & 1.182 &0.307 & new& \\
The-Croods-2 	 & 326 & 0.737 & 0.143 & 1.105 &0.308 & new& \\
Minions-1& 709 & 0.734 & 0.102 & 0.960 &0.325 & new& \\
KungFu-Panda-1 	 & 339 & 0.739 & 0.124 & 0.860 &0.329 & new& \\
Wall-E-2 	 & 274 & 0.708 & 0.153 & 1.083 &0.356 & new& \\
KungFu-Panda-2 	 & 374 & 0.687 & 0.079 & 0.903 &0.366 & new& \\
IceAge1 	 & 329 & 0.611 & 0.151 & 1.009 &0.469 & new& \\
insideout3 	 & 261 & 0.633 & 0.206 & 1.078 &0.474 & new& \\
IceAge2 	 & 175 & 0.631 & 0.177 & 1.041 &0.479 & new& \\
The-croods-3 	 & 122 & 0.651 & 0.225 & 1.098 &0.527 & new& \\
The-croods-1 	 & 208 & 0.544 & 0.115 & 0.978 &0.546 & new& \\
Minions-2& 220 & 0.606 & 0.247 & 0.997 &0.592 & new& \\
tom-jerry-2 	 & 251 & 0.526 & 0.185 & 0.922 &0.648 & new& \\
The-lion-king 	 & 251 & 0.472 & 0.203 & 1.007 &0.675 & new& \\
Ironman 	 & 166 & 0.489 & 0.132 & 1.053 &0.727 & OTB2015& \\
Bird1 	 & 408 & 0.205 & 0.065 & 0.995 &0.872 & OTB2015& \\
\bottomrule
% }

\end{longtable}

% \end{center}
% \vspace{-4mm}
% \end{table*}


==> tables/seq-info-v1.tex <==



% \begin{table*}[t]
% \begin{center}
% \caption{\textbf{ Detailed information about each sequence.} }
% \label{Tab:seq-info}
% \vspace{-2mm}
% \renewcommand\arraystretch{1.1}
% \setlength\tabcolsep{4pt}
 
\begin{longtable}{ll| ccccccc}
\caption{\textbf{ Detailed information of the 180 sequences.} Length: frame number of a sequence, Mean-IoU: mean IoU score obtained by the 15 methods given in the manuscript, STD-IoU: the standard deviation of the IoU scores, Var-density: appearance variation density, Quality: quality of a sequence. Source: where the sequence comes from (new indicates the sequence is newly collected).}
\vspace{-4mm}
\label{Tab:seq-info}\\
%  \resizebox{0.98\linewidth}{!}{
\toprule    
          &\multicolumn{1}{l|}{Sequence name}
          &\multirow{1}{*}{\tabincell{c}{Length}}
          &\multirow{1}{*}{\tabincell{c}{Mean-IoU}}
          &\multirow{1}{*}{\tabincell{c}{STD-IoU}}
          &\multirow{1}{*}{\tabincell{c}{Var-density}}
          &\multirow{1}{*}{\tabincell{c}{Quality}}
          &\multirow{1}{*}{\tabincell{c}{Source}}\\
        %   &\multirow{1}{*}{\tabincell{c}{Challenges}}\\
\midrule
\endfirsthead
\toprule    
          &\multicolumn{1}{l|}{Sequence name}
          &\multirow{1}{*}{\tabincell{c}{Length}}
          &\multirow{1}{*}{\tabincell{c}{Mean-IoU}}
          &\multirow{1}{*}{\tabincell{c}{STD-IoU}}
          &\multirow{1}{*}{\tabincell{c}{Var-density}}
          &\multirow{1}{*}{\tabincell{c}{Quality}}
          &\multirow{1}{*}{\tabincell{c}{Source}}\\
        %   &\multirow{1}{*}{\tabincell{c}{Challenges}}\\
\midrule
\endhead

\bottomrule
\endfoot

%--Human part
\multirow{20}{*}{\rotatebox{90}{\textbf{Human part}}}
&hand-piano 	     & 204 & 0.623 & 0.177 & 1.065 &0.570 & new\\
&foot-running 	 & 117 & 0.592 & 0.238 & 0.953 &0.577 & new\\
&helmet-football  & 284 & 0.485 & 0.103 & 1.039 &0.676 & new\\
&foot-dance   	 & 352 & 0.502 & 0.142 & 1.068 &0.680 & new\\
&helmet           & 125 & 0.565 & 0.302 & 1.090 &0.700 & new\\
&head-men's100 	 & 134 & 0.519 & 0.167 & 1.053 &0.718 & new\\
&foot-gait-1 	 & 245 & 0.454 & 0.116 & 0.956 &0.742 & new\\
&foot-gait-2 	 & 235 & 0.319 & 0.098 & 0.731 &0.863 & new\\
&head-breaking2 	 & 230 & 0.370 & 0.144 & 1.044 &0.865 & new\\
&head-swimming 	 & 175 & 0.371 & 0.138 & 0.995 &0.885 & new\\
&hand-ASL         & 398 & 0.424 & 0.193 & 0.977 &0.891 & new\\
&Soccer 	         & 392 & 0.335 & 0.113 & 0.771 &0.893 & OTB2015~\cite{OTB2015}\\
&foot-ballet 	 & 336 & 0.066 & 0.041 & 1.056 &0.897 & new\\
&hand-language2 	 & 144 & 0.311 & 0.117 & 1.106 &0.904 & new\\
&hand-dance-1 	 & 357 & 0.264 & 0.160 & 1.051 &0.969 & new\\
&hand-dance-2 	 & 342 & 0.310 & 0.175 & 1.082 &0.971 & new\\
&foot-breaking 	 & 193 & 0.181 & 0.107 & 1.121 &1.022 & new\\
&hat-2 	         & 1461 & 0.361 & 0.216 & 1.031 &1.025 & LaSOT~\cite{LaSOT}\\
&head-boxing 	 & 297 & 0.247 & 0.264 & 1.081 &1.049 & new\\
&hand-9 	         & 1733 & 0.144 & 0.085 & 0.870 &1.087 & LaSOT\\ \midrule
%--Sport ball
 \multirow{20}{*}{\rotatebox{90}{\textbf{Sport ball}}}
&soccer 2 	 & 77 & 0.715 & 0.191 & 1.160 &0.420 & new&\\
&basketball-3 & 130 & 0.619 & 0.136 & 1.128 &0.444 & new\\
&rugby 1 	 & 109 & 0.610 & 0.226 & 0.976 &0.572 & new\\
&rugby-kick2 	 & 100 & 0.219 & 0.045 & 1.074 &0.611 & new\\
&basketball-1 	 & 118 & 0.599 & 0.304 & 1.023 &0.629 & new\\
&valleyball1 	 & 281 & 0.547 & 0.322 & 1.009 &0.832 & new\\
&golf 2 	 & 153 & 0.395 & 0.189 & 1.091 &0.861 & new\\
&volleyball 	 & 142 & 0.131 & 0.162 & 1.132 &0.865 & new\\
&snooker-2 	 & 88 & 0.195 & 0.285 & 0.999 &0.881 & new\\
&rugby 2 	 & 166 & 0.390 & 0.191 & 0.979 &0.886 & new\\
&nine-ball-pool 	 & 210 & 0.456 & 0.320 & 0.940 &0.886 & new\\
&basketball-2 	 & 123 & 0.385 & 0.256 & 1.018 &0.913 & new\\
&snooker-1 	 & 98 & 0.310 & 0.330 & 1.075 &0.934 & new\\
&pingpong-8 	 & 296 & 0.186 & 0.129 & 1.046 &0.987 & NFS~\cite{NFS}\\
&golf 1 	 & 138 & 0.353 & 0.292 & 0.950 &1.043 & new\\
&pingpong2 	 & 103 & 0.230 & 0.246 & 0.942 &1.064 & new\\
&pingpong1 	 & 107 & 0.223 & 0.290 & 1.038 &1.099 & new\\
&soccer 	 & 225 & 0.303 & 0.262 & 1.079 &1.112 & new\\
&billiard-6 	 & 771 & 0.349 & 0.365 & 0.990 &1.114 & NFS\\
&volleyball-13 	 & 2004 & 0.255 & 0.295 & 1.166 &1.292 & LaSOT\\\midrule
%--3D-object
 \multirow{8}{*}{\rotatebox{90}{\textbf{3D-object}}}
&toy-car1 	 & 201 & 0.759 & 0.124 & 0.840 &0.299 & new&\\
&yoyo-inhand-night 	 & 321 & 0.749 & 0.054 & 1.013 &0.320 & new\\
&toy-car3 	 & 409 & 0.662 & 0.088 & 1.095 &0.376 & new\\
&toy-fight 	 & 256 & 0.715 & 0.172 & 1.159 &0.396 & new\\
&toy-train 	 & 380 & 0.653 & 0.112 & 1.158 &0.405 & new\\
&box-inhand 	 & 438 & 0.667 & 0.137 & 1.022 &0.416 & new\\
&cubes-inhand 	 & 149 & 0.626 & 0.180 & 1.063 &0.460 & new\\
&bottle-flip2 	 & 136 & 0.619 & 0.218 & 1.010 &0.564 & new\\
 \multirow{12}{*}{\rotatebox{90}{\textbf{3D-object}}}
&toy-helicopter 	 & 400 & 0.559 & 0.152 & 1.006 &0.612 & new\\
&cup-inhand 	 & 418 & 0.142 & 0.054 & 0.915 &0.718 & new\\
&toy-car2 	 & 268 & 0.461 & 0.215 & 0.714 &0.786 & new\\
&bottle-flip 	 & 127 & 0.425 & 0.245 & 1.071 &0.812 & new\\
&toy-box 	 & 479 & 0.278 & 0.175 & 1.114 &0.882 & new\\
&toy-inhand-yoyo 	 & 404 & 0.461 & 0.290 & 0.986 &0.922 & new\\
&juggling-2 	 & 168 & 0.121 & 0.055 & 1.031 &0.935 & new\\
&robot-5 	 & 2267 & 0.290 & 0.159 & 0.981 &0.947 & LaSOT\\
&juggling-1 	 & 211 & 0.094 & 0.074 & 1.084 &1.006 & new\\
&shuffletable-2 	 & 372 & 0.262 & 0.267 & 0.979 &1.063 & NFS\\
&airtable-3 	 & 482 & 0.152 & 0.176 & 0.962 &1.083 & NFS\\
&kite-15 	 & 2064 & 0.156 & 0.202 & 0.996 &1.290 & LaSOT\\\midrule
%--Animal
\multirow{20}{*}{\rotatebox{90}{\textbf{Animal}}}
&Panda-head 	 & 312 & 0.746 & 0.076 & 1.000 &0.303 & new\\
&leopard 	 & 221 & 0.710 & 0.114 & 1.100 &0.366 & new\\
&horse-zebra 	 & 286 & 0.596 & 0.099 & 1.174 &0.483 & new\\
&lion-running 	 & 367 & 0.666 & 0.215 & 1.061 &0.494 & new\\
&air-sea-dolphin 	 & 342 & 0.610 & 0.156 & 1.001 &0.494 & new\\
&cat-eat 	 & 381 & 0.564 & 0.074 & 0.919 &0.507 & new\\
&butterfly-2 	 & 302 & 0.647 & 0.162 & 0.965 &0.536 & new\\
&panda-funny 	 & 383 & 0.567 & 0.164 & 0.976 &0.597 & new\\
&bird-flying 	 & 440 & 0.574 & 0.174 & 0.894 &0.648 & new\\
&dogs 	 & 395 & 0.402 & 0.148 & 1.041 &0.754 & new\\
&bull 	 & 131 & 0.401 & 0.210 & 0.781 &0.772 & new\\
&bird-sea 	 & 378 & 0.384 & 0.197 & 0.990 &0.873 & new\\
&fish2 	 & 371 & 0.355 & 0.223 & 0.975 &0.915 & new\\
&bee-group 	 & 431 & 0.377 & 0.252 & 1.129 &0.958 & new\\
&squirrel-13 	 & 1927 & 0.214 & 0.099 & 1.112 &1.013 & LaSOT\\
&dogs2 	 & 394 & 0.320 & 0.194 & 1.182 &1.026 & new\\
&dog-2 	 & 594 & 0.129 & 0.202 & 1.041 &1.084 & NFS\\
&shark-2 	 & 3441 & 0.235 & 0.147 & 1.091 &1.113 & LaSOT\\
&butterfly-1 	 & 305 & 0.270 & 0.249 & 0.968 &1.157 & new\\
&goldfish-3 	 & 2163 & 0.225 & 0.168 & 0.973 &1.204 & LaSOT\\\midrule
%--UAV

&air-ground-f1 	 & 241 & 0.693 & 0.180 & 0.938 &0.361 & new\\
\multirow{19}{*}{\rotatebox{90}{\textbf{UAV}}}
&air-ground-bike-2 	 & 361 & 0.729 & 0.208 & 1.125 &0.402 & new\\
&air-ground-lake 	 & 321 & 0.668 & 0.184 & 1.091 &0.424 & new\\
&ground-air-drone1 	 & 584 & 0.658 & 0.194 & 0.940 &0.494 & new\\
&ground-air-drone2 	 & 347 & 0.592 & 0.130 & 1.034 &0.519 & new\\
&skating-uav 	 & 319 & 0.602 & 0.111 & 1.113 &0.520 & new\\
&air-ground-skiing 	 & 462 & 0.527 & 0.156 & 0.954 &0.671 & new\\
&air-ground-car 	 & 554 & 0.553 & 0.214 & 1.055 &0.677 & new\\
&air-air-rocket3 	 & 158 & 0.576 & 0.270 & 1.053 &0.685 & new\\
&air-air-rocket4 	 & 926 & 0.422 & 0.180 & 0.825 &0.800 & new\\
&air-air-drone1 	 & 463 & 0.364 & 0.156 & 1.107 &0.870 & new\\
&air-air-eagle 	 & 387 & 0.450 & 0.296 & 0.965 &0.954 & new\\
&uav0000080-01680-s 	 & 1201 & 0.335 & 0.211 & 1.123 &0.986 & VisDrone~\cite{VisDrone}\\
&uav0000070-04877-s 	 & 332 & 0.278 & 0.229 & 0.971 &0.997 & VisDrone\\
&person19-3 	 & 1567 & 0.297 & 0.216 & 0.898 &1.002 & UAV\\
&car15 	 & 469 & 0.387 & 0.279 & 1.039 &1.043 & UAV~\cite{UAV123}\\
&uav0000085-00000-s 	 & 1645 & 0.264 & 0.233 & 0.949 &1.086 & VisDrone\\
&uav0000221-10400-s 	 & 2970 & 0.159 & 0.226 & 1.049 &1.120 & VisDrone\\
&uav4 	 & 157 & 0.204 & 0.192 & 0.946 &1.125 & UAV\\
&drone-7 	 & 2708 & 0.313 & 0.257 & 1.045 &1.196 & LaSOT\\\midrule
%--Human body
 \multirow{20}{*}{\rotatebox{90}{\textbf{Human body}}}
&mountain-biker 	 & 226 & 0.656 & 0.135 & 1.161 &0.408 & new&\\
&long-jump 	 & 298 & 0.719 & 0.163 & 1.104 &0.410 & new\\
&polo 	 & 301 & 0.637 & 0.064 & 1.119 &0.419 & new\\
&beark-dancer 	 & 357 & 0.702 & 0.135 & 1.054 &0.425 & new\\
&pole-vault 	 & 199 & 0.642 & 0.116 & 1.032 &0.478 & new\\
&high-jumper 	 & 300 & 0.632 & 0.153 & 1.207 &0.507 & new\\
&ski-jumper 	 & 315 & 0.575 & 0.144 & 1.110 &0.517 & new\\
&pedestrian 	 & 147 & 0.523 & 0.099 & 1.003 &0.518 & new\\
&skater2 	 & 319 & 0.602 & 0.111 & 0.985 &0.520 & new\\
&runner1 	 & 192 & 0.559 & 0.145 & 1.168 &0.642 & new\\
&pair-diving 	 & 60 & 0.534 & 0.196 & 1.083 &0.661 & new\\
&gymnastics3 	 & 380 & 0.569 & 0.224 & 1.158 &0.734 & new\\
&gymnastics2 	 & 300 & 0.574 & 0.311 & 1.078 &0.753 & new\\
&Human3 	 & 1698 & 0.506 & 0.294 & 0.938 &0.908 & OTB2015\\
&parkour 	 & 58 & 0.146 & 0.159 & 1.066 &0.910 & NFS\\
&basketball-7 	 & 240 & 0.327 & 0.227 & 1.175 &0.947 & NFS\\
&basketball-005 	 & 196 & 0.218 & 0.138 & 1.105 &0.975 & NUS-PRO~\cite{NUS-PRO}\\
&Skydiving 	 & 196 & 0.213 & 0.147 & 1.097 &0.993 & NFS\\
&handball-004 	 & 218 & 0.202 & 0.174 & 1.077 &0.994 & NUS-PRO\\
&soccer-006 	 & 387 & 0.143 & 0.214 & 1.059 &1.017 & NUS-PRO\\\midrule
%--Vehicle
\multirow{20}{*}{\rotatebox{90}{\textbf{Vehicle}}}
&car-night 	 & 422 & 0.793 & 0.039 & 1.110 &0.246 & new&\\
&bike-wild 	 & 205 & 0.763 & 0.122 & 1.094 &0.284 & new\\
&bike-auto 	 & 390 & 0.725 & 0.120 & 0.970 &0.313 & new\\
&car-drifting 	 & 460 & 0.761 & 0.246 & 1.062 &0.338 & new\\
&cars-racing 	 & 248 & 0.657 & 0.084 & 1.144 &0.393 & new\\
&motor-racing 	 & 392 & 0.651 & 0.136 & 1.135 &0.418 & new\\
&train-night 	 & 449 & 0.699 & 0.251 & 1.015 &0.445 & new\\
&plane-takingoff 	 & 472 & 0.572 & 0.103 & 1.192 &0.488 & new\\
&board 	 & 392 & 0.612 & 0.134 & 1.070 &0.491 & new\\
&train-1 	 & 317 & 0.556 & 0.121 & 1.167 &0.514 & new\\
&boat-racing2 	 & 349 & 0.620 & 0.228 & 1.035 &0.551 & new\\
&boat-racing1 	 & 450 & 0.597 & 0.219 & 1.052 &0.615 & new\\
&helicopter1 	 & 425 & 0.597 & 0.249 & 0.960 &0.624 & new\\
&truck 	 & 402 & 0.564 & 0.171 & 0.892 &0.627 & new\\
&jet-2 	 & 388 & 0.486 & 0.247 & 1.121 &0.733 & new\\
&suv 	 & 457 & 0.239 & 0.090 & 1.106 &0.901 & new\\
&train-highspeed 	 & 407 & 0.302 & 0.219 & 1.058 &0.973 & new\\
&bike3 	 & 433 & 0.302 & 0.203 & 1.081 &0.995 & UAV\\
&racing-20 	 & 2812 & 0.167 & 0.174 & 0.996 &1.088 & LaSOT\\
&motorcycle-18 	 & 2382 & 0.209 & 0.254 & 1.060 &1.243 & LaSOT\\\midrule
%--Sign and logo
\multirow{8}{*}{\rotatebox{90}{\textbf{Sign-and-logo}}}
&led-snowy-coke 	 & 350 & 0.837 & 0.069 & 1.173 &0.166 & new\\
&sign-night-yellow 	 & 267 & 0.827 & 0.065 & 1.058 &0.200 & new\\
&sign-day-tunnel 	 & 294 & 0.797 & 0.073 & 1.216 &0.239 & new\\
&sign-night-direction 	 & 305 & 0.786 & 0.054 & 1.049 &0.257 & new\\
&sign-night-led 	 & 399 & 0.758 & 0.065 & 0.979 &0.290 & new\\
&sign-night-speed 	 & 219 & 0.742 & 0.056 & 1.164 &0.295 & new\\
&text-mlines 	 & 225 & 0.735 & 0.229 & 1.144 &0.356 & new\\
&sign-day-light1 	 & 348 & 0.715 & 0.128 & 1.036 &0.364 & new\\
\multirow{12}{*}{\rotatebox{90}{\textbf{Sign-and-logo}}}
&sign-snow-street 	 & 385 & 0.677 & 0.078 & 1.106 &0.387 & new\\
&sign-day-direction2 	 & 226 & 0.659 & 0.124 & 0.990 &0.414 & new\\
&sign-day-light2 	 & 187 & 0.661 & 0.175 & 1.054 &0.458 & new\\
&sign-street-speed 	 & 235 & 0.621 & 0.216 & 1.031 &0.568 & new\\
&sign-night-light4 	 & 185 & 0.467 & 0.124 & 1.117 &0.574 & new\\
&text-coffee 	 & 188 & 0.588 & 0.279 & 1.014 &0.577 & new\\
&sign-night-light 	 & 353 & 0.492 & 0.126 & 1.108 &0.716 & new\\
&sign-night-light3 	 & 357 & 0.423 & 0.151 & 0.915 &0.740 & new\\
&clifBar 	 & 472 & 0.484 & 0.182 & 1.011 &0.786 & OTB2015\\
&sign-groundstop 	 & 77 & 0.286 & 0.206 & 0.950 &0.868 & new\\
&led-night-text 	 & 295 & 0.285 & 0.293 & 1.036 &1.064 & new\\
&licenseplate-12 	 & 2554 & 0.267 & 0.179 & 1.007 &1.076 & LaSOT\\\midrule
%--Cartoon
 \multirow{20}{*}{\rotatebox{90}{\textbf{Cartoon}}}
&insideout-face 	 & 299 & 0.803 & 0.045 & 0.935 &0.223 & new&\\
&Wall-E-1 	 & 320 & 0.744 & 0.093 & 1.123 &0.287 & new\\
&tom-jerry-1 	 & 227 & 0.744 & 0.042 & 1.143 &0.297 & new\\
&Totoro1 	 & 379 & 0.734 & 0.093 & 1.012 &0.303 & new\\
&Totoro0 	 & 351 & 0.747 & 0.221 & 1.182 &0.307 & new\\
&The-Croods-2 	 & 326 & 0.737 & 0.143 & 1.105 &0.308 & new\\
&Minions-1& 709 & 0.734 & 0.102 & 0.960 &0.325 & new\\
&KungFu-Panda-1 	 & 339 & 0.739 & 0.124 & 0.860 &0.329 & new\\
&Wall-E-2 	 & 274 & 0.708 & 0.153 & 1.083 &0.356 & new\\
&KungFu-Panda-2 	 & 374 & 0.687 & 0.079 & 0.903 &0.366 & new\\
&IceAge1 	 & 329 & 0.611 & 0.151 & 1.009 &0.469 & new\\
&insideout3 	 & 261 & 0.633 & 0.206 & 1.078 &0.474 & new\\
&IceAge2 	 & 175 & 0.631 & 0.177 & 1.041 &0.479 & new\\
&The-croods-3 	 & 122 & 0.651 & 0.225 & 1.098 &0.527 & new\\
&The-croods-1 	 & 208 & 0.544 & 0.115 & 0.978 &0.546 & new\\
&Minions-2& 220 & 0.606 & 0.247 & 0.997 &0.592 & new\\
&tom-jerry-2 	 & 251 & 0.526 & 0.185 & 0.922 &0.648 & new\\
&The-lion-king 	 & 251 & 0.472 & 0.203 & 1.007 &0.675 & new\\
&Ironman 	 & 166 & 0.489 & 0.132 & 1.053 &0.727 & OTB2015\\
&Bird1 	 & 408 & 0.205 & 0.065 & 0.995 &0.872 & OTB2015\\
\bottomrule
% }

\end{longtable}

% \end{center}
% \vspace{-4mm}
% \end{table*}

